Self-Supervised Transformers for fMRI representation

We present TFF, which is a Transformer framework for the analysis of functional Magnetic Resonance Imaging (fMRI) data. TFF employs a two-phase training approach. First, self-supervised training is applied to a collection of fMRI scans, where the model is trained to reconstruct 3D volume data. Second, the pre-trained model is fine-tuned on specific tasks, utilizing ground truth labels. Our results show state-of-the-art performance on a variety of fMRI tasks, including age and gender prediction, as well as schizophrenia recognition. Our code for the training, network architecture, and results is attached as supplementary material.

==> many-authors-hack.tex <==
%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}
